Conflict-driven Hybrid Observer-based Anomaly Detection

This paper presents an anomaly detection method using a hybrid observer -- which consists of a discrete state observer and a continuous state observer. We focus our attention on anomalies caused by intelligent attacks, which may bypass existing anomaly detection methods because neither the event sequence nor the observed residuals appear to be anomalous. Based on the relation between the continuous and discrete variables, we define three conflict types and give the conditions under which the detection of the anomalies is guaranteed. We call this method conflict-driven anomaly detection. The effectiveness of this method is demonstrated mathematically and illustrated on a Train-Gate (TG) system.

==> sec-motivation.tex <==
\section{Motivational Example} \label{sec-motivation}
Here, we consider the Tran-Gait (TG) system as the motivational example. This system includes a train, a gate at the road to stop the traffic and two sensors that sense the arrival and departure of the train. The schematic of this system is illustrated in Fig. \ref{fig-TGCsys}. 
\begin{figure}[!h]
	\centering
	\includegraphics[width=3.2in]{TrainGateControllerSys.PNG}
	\caption{TG Schematic}
	\label{fig-TGCsys}
\end{figure} 

The TG system can be represented with a hybrid model. The train with an internal controller for the train speed is the continuous system. 
An external controller changes the reference train speed based on the measured train position such that the train passes the gate with a lower speed. 
The gate is a discrete system, which is raised or lowered by a controller using two presence sensors located on both sides of the road. 
The first sensor detects the arrival of the train setting the gate to the down position, and the second sensor indicates the departure of the train, which sets the gate to the up position.
Two monitors are used to detect anomalies. Assume that two independent monitors are installed for the detection of anomalies. One monitor detects anomalies in the continuous train system, by comparing the estimates of the continuous outputs with the observed ones. The second monitor detects anomalies in the discrete gate system by comparing the expected discrete event sequence obtained from model with the observed one.  


However, an attacker can launch an attack to cause an anomaly bypassing both monitors. For example, an anomalous ramp signal could be added to the measured train position without increasing the difference between the estimated and the observed outputs. Thus, the monitor for the continuous train system cannot detect it. The monitor for the discrete gate system cannot detect it because the discrete state sequence is not changed by this anomaly.
The drifted measured position can make the train pass the gate with a high speed, causing insufficient time of lowering the gate. A driver may pass the gate, causing a severe accident. 


